Lara Mini Base: Language Diversity as a Resource, Not a Trade-off

General-purpose language models are trained mostly on English: over open models we review, at most, non-English pretraining data makes up only a 12% share. Models built for European languages give them far more, but score well below general-purpose models of the same size. A common concern is that, in small models, languages compete for capacity. We present Lara Mini base, a model trained from scratch on 6T tokens in English and 44 other languages, which together cover all 24 official languages of the European Union. As training progresses, the 44 other languages together come to outweigh English. To give these languages enough capacity at low cost, Lara Mini base uses a mixture of experts architecture with 7.2B total and 0.6B active parameters. Among open base models with up to 2B active parameters, it achieves the highest average score across standard English, multilingual, math, and code benchmarks, ahead of models trained on 4 to 6 times as many tokens. Its margin is largest on multilingual benchmarks in the languages it supports and on math benchmarks. It supports contexts of up to 128k tokens. We find that our MoE architecture reduces capacity competition between languages. For a single user on one GPU, without quantization, it generates text at least 1.8 times faster than any model with a higher average score. We release the weights of Lara Mini base under the CC BY-NC-SA 4.0 license. In addition, we will release T-HellaSwag, a higher-quality machine translation of the commonsense reasoning benchmark HellaSwag into 110 language variants.

==> figures/logos/huggingface-logo.tex <==
\definecolor{lrhflogoa}{HTML}{FFD21E}
\definecolor{lrhflogob}{HTML}{FF9D0B}
\definecolor{lrhflogoc}{HTML}{3A3B45}
\definecolor{lrhflogod}{HTML}{FF323D}
\newcommand{\HuggingFaceLogo}[1]{%
  \begingroup
  \pgfmathsetmacro{\hflogoscale}{(#1)/88}%
  \begin{tikzpicture}[x=1pt, y=1pt, xscale=\hflogoscale, yscale=-\hflogoscale]
    \useasboundingbox (0,0) rectangle (95,88);
    \fill[lrhflogoa] svg {M47.21,76.5 C66.402,76.5 81.96,60.942 81.96,41.75 C81.96,22.558 66.402,7 47.21,7 C28.018,7 12.46,22.558 12.46,41.75 C12.46,60.942 28.018,76.5 47.21,76.5 Z};
    \fill[lrhflogob] svg {M81.96,41.75 C81.96,22.558 66.402,7 47.21,7 C28.018,7 12.46,22.558 12.46,41.75 C12.46,60.942 28.018,76.5 47.21,76.5 C66.402,76.5 81.96,60.942 81.96,41.75 Z M8.46,41.75 C8.46,20.349 25.809,3 47.21,3 C68.611,3 85.96,20.349 85.96,41.75 C85.96,63.151 68.611,80.5 47.21,80.5 C25.809,80.5 8.46,63.151 8.46,41.75 Z};
    \fill[lrhflogoc] svg {M58.5,32.3 C59.78,32.74 60.28,35.36 61.57,34.68 C63.356,33.732 64.395,31.8 64.203,29.787 C64.01,27.774 62.623,26.075 60.689,25.483 C58.755,24.891 56.655,25.522 55.368,27.082 C54.081,28.642 53.861,30.824 54.81,32.61 C55.42,33.76 57.36,31.89 58.51,32.29 Z M34.95,32.3 C33.67,32.74 33.16,35.36 31.88,34.68 C30.094,33.732 29.055,31.8 29.247,29.787 C29.44,27.774 30.827,26.075 32.761,25.483 C34.695,24.891 36.795,25.522 38.082,27.082 C39.369,28.642 39.589,30.824 38.64,32.61 C38.03,33.76 36.08,31.89 34.94,32.29 Z};
    \fill[lrhflogod] svg {M46.96,56.29 C56.79,56.29 59.96,47.53 59.96,43.03 C59.96,40.69 58.39,41.43 55.87,42.67 C53.54,43.82 50.41,45.41 46.97,45.41 C39.78,45.41 33.97,38.53 33.97,43.03 C33.97,47.53 37.13,56.29 46.97,56.29 Z};
    \fill[lrhflogoc, even odd rule] svg {M39.43,54 C40.497,51.832 42.417,50.206 44.73,49.51 C45.13,49.39 45.54,50.08 45.97,50.79 C46.37,51.47 46.79,52.16 47.21,52.16 C47.66,52.16 48.11,51.48 48.54,50.81 C48.99,50.11 49.43,49.43 49.86,49.56 C52.008,50.242 53.803,51.739 54.86,53.73 C58.59,50.79 59.96,45.99 59.96,43.03 C59.96,40.69 58.39,41.43 55.87,42.67 L55.73,42.74 C53.42,43.89 50.34,45.41 46.96,45.41 C43.58,45.41 40.51,43.89 38.19,42.74 C35.59,41.45 33.96,40.64 33.96,43.03 C33.96,46.08 35.42,51.09 39.43,54 Z};
    \fill[lrhflogob] svg {M70.71,37 C72.505,37 73.96,35.545 73.96,33.75 C73.96,31.955 72.505,30.5 70.71,30.5 C68.915,30.5 67.46,31.955 67.46,33.75 C67.46,35.545 68.915,37 70.71,37 Z M24.21,37 C26.005,37 27.46,35.545 27.46,33.75 C27.46,31.955 26.005,30.5 24.21,30.5 C22.415,30.5 20.96,31.955 20.96,33.75 C20.96,35.545 22.415,37 24.21,37 Z M17.52,48 C15.9,48 14.46,48.66 13.45,49.87 C12.589,50.934 12.119,52.261 12.12,53.63 C11.49,53.441 10.837,53.34 10.18,53.33 C8.63,53.33 7.23,53.92 6.24,54.99 C4.424,56.875 4.097,59.743 5.44,61.99 C4.555,62.713 3.927,63.702 3.65,64.81 C3.41,65.71 3.17,67.61 4.45,69.55 C3.475,71.049 3.335,72.944 4.08,74.57 C5.1,76.89 7.65,78.71 12.6,80.67 C15.67,81.89 18.49,82.67 18.51,82.68 C22.072,83.667 25.744,84.204 29.44,84.28 C35.3,84.28 39.49,82.48 41.9,78.94 C45.78,73.25 45.23,68.04 40.2,63.02 C37.43,60.24 35.58,56.15 35.2,55.25 C34.42,52.59 32.36,49.63 28.95,49.63 C27.109,49.659 25.396,50.575 24.35,52.09 C23.35,50.83 22.37,49.84 21.49,49.27 C20.316,48.475 18.938,48.034 17.52,48 Z M17.52,52 C18.03,52 18.66,52.22 19.34,52.65 C21.48,54.01 25.59,61.08 27.1,63.83 C27.6,64.75 28.47,65.14 29.24,65.14 C30.79,65.14 31.99,63.61 29.39,61.66 C25.47,58.73 26.84,53.94 28.71,53.65 C28.79,53.63 28.88,53.63 28.95,53.63 C30.65,53.63 31.4,56.56 31.4,56.56 C31.4,56.56 33.6,62.08 37.38,65.86 C41.15,69.63 41.35,72.66 38.6,76.69 C36.72,79.44 33.13,80.27 29.44,80.27 C25.63,80.27 21.71,79.37 19.52,78.81 C19.41,78.78 6.07,75.01 7.76,71.81 C8.04,71.27 8.51,71.05 9.1,71.05 C11.48,71.05 15.8,74.59 17.67,74.59 C18.08,74.59 18.37,74.42 18.5,73.99 C19.29,71.14 6.44,69.94 7.52,65.82 C7.72,65.09 8.23,64.8 8.96,64.8 C12.1,64.8 19.16,70.33 20.64,70.33 C20.75,70.33 20.84,70.3 20.88,70.23 C21.62,69.03 21.21,68.19 15.98,65.03 C10.77,61.87 7.1,59.97 9.18,57.7 C9.42,57.44 9.76,57.32 10.18,57.32 C13.35,57.32 20.84,64.14 20.84,64.14 C20.84,64.14 22.86,66.24 24.09,66.24 C24.37,66.24 24.61,66.14 24.77,65.86 C25.63,64.4 16.71,57.64 16.21,54.85 C15.87,52.95 16.45,52 17.52,52 Z};
    \fill[lrhflogoa] svg {M38.6,76.69 C41.35,72.65 41.15,69.62 37.38,65.85 C33.6,62.08 31.4,56.55 31.4,56.55 C31.4,56.55 30.58,53.35 28.71,53.65 C26.84,53.95 25.47,58.73 29.39,61.66 C33.3,64.59 28.61,66.58 27.1,63.83 C25.6,61.08 21.48,54.01 19.34,52.65 C17.21,51.3 15.71,52.05 16.21,54.85 C16.71,57.64 25.64,64.4 24.77,65.85 C23.9,67.32 20.84,64.14 20.84,64.14 C20.84,64.14 11.27,55.43 9.18,57.7 C7.1,59.97 10.77,61.87 15.98,65.03 C21.21,68.19 21.62,69.03 20.88,70.23 C20.13,71.43 8.6,61.7 7.52,65.83 C6.44,69.94 19.29,71.13 18.5,73.98 C17.7,76.83 9.44,68.6 7.76,71.8 C6.06,75.01 19.41,78.78 19.52,78.81 C23.82,79.93 34.77,82.3 38.6,76.69 Z};
    \fill[lrhflogob] svg {M77.4,48 C79.02,48 80.47,48.66 81.47,49.87 C82.331,50.934 82.801,52.261 82.8,53.63 C83.433,53.44 84.089,53.339 84.75,53.33 C86.3,53.33 87.7,53.92 88.69,54.99 C90.506,56.875 90.833,59.743 89.49,61.99 C90.371,62.714 90.996,63.703 91.27,64.81 C91.51,65.71 91.75,67.61 90.47,69.55 C91.445,71.049 91.585,72.944 90.84,74.57 C89.82,76.89 87.27,78.71 82.33,80.67 C79.25,81.89 76.43,82.67 76.41,82.68 C72.848,83.667 69.176,84.204 65.48,84.28 C59.62,84.28 55.43,82.48 53.02,78.94 C49.14,73.25 49.69,68.04 54.72,63.02 C57.5,60.24 59.35,56.15 59.73,55.25 C60.51,52.59 62.56,49.63 65.97,49.63 C67.811,49.659 69.524,50.575 70.57,52.09 C71.57,50.83 72.55,49.84 73.44,49.27 C74.611,48.477 75.986,48.036 77.4,48 Z M77.4,52 C76.89,52 76.27,52.22 75.58,52.65 C73.45,54.01 69.33,61.08 67.82,63.83 C67.405,64.63 66.581,65.134 65.68,65.14 C64.14,65.14 62.93,63.61 65.54,61.66 C69.45,58.73 68.08,53.94 66.21,53.65 C66.131,53.637 66.05,53.63 65.97,53.63 C64.27,53.63 63.52,56.56 63.52,56.56 C63.52,56.56 61.32,62.08 57.55,65.86 C53.77,69.63 53.57,72.66 56.33,76.69 C58.2,79.44 61.8,80.27 65.48,80.27 C69.3,80.27 73.21,79.37 75.41,78.81 C75.51,78.78 88.86,75.01 87.17,71.81 C86.88,71.27 86.42,71.05 85.83,71.05 C83.45,71.05 79.12,74.59 77.26,74.59 C76.84,74.59 76.55,74.42 76.43,73.99 C75.63,71.14 88.48,69.94 87.4,65.82 C87.21,65.09 86.7,64.8 85.96,64.8 C82.82,64.8 75.76,70.33 74.28,70.33 C74.18,70.33 74.09,70.3 74.05,70.23 C73.31,69.03 73.71,68.19 78.93,65.03 C84.16,61.87 87.83,59.97 85.73,57.7 C85.5,57.44 85.16,57.32 84.75,57.32 C81.57,57.32 74.08,64.14 74.08,64.14 C74.08,64.14 72.06,66.24 70.84,66.24 C70.56,66.253 70.296,66.105 70.16,65.86 C69.29,64.4 78.21,57.64 78.71,54.85 C79.05,52.95 78.47,52 77.4,52 Z};
    \fill[lrhflogoa] svg {M56.33,76.69 C53.58,72.65 53.77,69.62 57.55,65.85 C61.32,62.08 63.52,56.55 63.52,56.55 C63.52,56.55 64.34,53.35 66.22,53.65 C68.08,53.95 69.45,58.73 65.54,61.66 C61.62,64.59 66.32,66.58 67.82,63.83 C69.33,61.08 73.45,54.01 75.58,52.65 C77.71,51.3 79.22,52.05 78.71,54.85 C78.21,57.64 69.29,64.4 70.16,65.85 C71.02,67.32 74.08,64.14 74.08,64.14 C74.08,64.14 83.66,55.43 85.74,57.7 C87.82,59.97 84.16,61.87 78.94,65.03 C73.71,68.19 73.31,69.03 74.04,70.23 C74.79,71.43 86.32,61.7 87.4,65.83 C88.48,69.94 75.64,71.13 76.43,73.98 C77.23,76.83 85.48,68.6 87.17,71.8 C88.86,75.01 75.52,78.78 75.41,78.81 C71.1,79.93 60.15,82.3 56.33,76.69 Z};
  \end{tikzpicture}%
  \endgroup}


==> figures/logos/translated-logo.tex <==
\newcommand{\TranslatedLogo}[2][black]{%
  \begingroup
  \pgfmathsetmacro{\tlogoscale}{(#2)/40}%
  \begin{tikzpicture}[x=1pt, y=1pt, xscale=\tlogoscale, yscale=-\tlogoscale]
    \useasboundingbox (0,0) rectangle (192,40);
    \fill[#1] svg {M60.4556937,28.0640641 C59.4521011,28.8019644 58.2291003,29.1829227 56.9824984,29.1459459 C55.2051224,29.1459459 53.8439674,28.562963 53.0452731,27.2904905 C52.544683,26.5421421 52.350634,25.6564565 52.350634,24.2438438 L52.350634,16.6286286 L49.8983051,16.6286286 L49.8983051,14.2770771 L52.3421971,14.2770771 L52.3421971,10.3727728 L55.4357313,10.3727728 L55.4357313,14.2770771 L59.9354175,14.2770771 L59.9354175,16.6286286 L55.4357313,16.6286286 L55.4357313,24.2718719 C55.4357313,25.7377377 56.1303704,26.43003 57.404344,26.43003 C58.0709834,26.435647 58.7189682,26.2108071 59.2379661,25.7937938 L60.4556937,28.0640641 Z};
    \fill[#1] svg {M71.0805775,17.4974975 C70.5723573,17.2113672 69.999385,17.0589622 69.4156937,17.0546547 C67.5539485,17.0546547 65.9143754,18.6606607 65.9143754,21.427027 L65.9143754,28.8208208 L62.8574011,28.8208208 L62.8574011,14.2770771 L65.9284369,14.2770771 L65.9284369,16.6286286 C66.901494,15.1067067 68.3442059,13.9995996 70.0400251,13.9995996 C70.721617,13.9836317 71.3943033,14.1563287 71.9833271,14.4984985 L71.0805775,17.4974975 Z};
    \fill[#1] svg {M85.4430132,29.0338338 C84.0818581,29.0338338 82.8303829,28.3975976 82.5266541,26.8728729 C81.331425,28.590991 79.388123,29.1459459 77.6641808,29.1459459 C74.6634526,29.1459459 72.6639046,27.5119119 72.6639046,24.6614615 C72.6639046,21.0626627 75.8586817,20.5077077 78.3588198,20.233033 C80.47086,20.0116116 82.0541871,19.8182182 82.0541871,18.4056056 C82.0541871,16.992993 80.442737,16.5501502 79.0815819,16.5501502 C77.4492225,16.568857 75.8608353,17.0799188 74.5256497,18.016016 L73.3022976,15.7205205 C75.0794342,14.5436373 77.1701559,13.9255699 79.3037539,13.9463463 C82.7488261,13.9463463 85.1645951,15.3309309 85.1645951,18.8204204 L85.1645951,25.4378378 C85.1645951,26.3795796 85.4711362,26.7663664 86.1938983,26.7663664 C86.4748413,26.7777816 86.753403,26.7108031 86.9982172,26.572973 L87.3328814,28.6778779 C86.7326289,28.9195298 86.0903542,29.0405019 85.4430132,29.0338338 Z M82.0823101,21.0878879 C81.238619,22.1389389 79.998393,22.1389389 78.443189,22.3883884 C76.8879849,22.6378378 75.7461896,23.0806807 75.7461896,24.6026026 C75.7461896,26.1245245 76.9132957,26.7635636 78.4150659,26.7635636 C80.3302448,26.7635636 82.0710609,25.7377377 82.0710609,23.3021021 L82.0823101,21.0878879 Z};
    \fill[#1] svg {M89.2705587,28.8124124 L89.2705587,14.2770771 L92.327533,14.2770771 L92.327533,16.4072072 C93.5199498,14.8292292 95.1398368,13.9435435 97.1084495,13.9435435 C100.303227,13.9435435 102.136849,16.0764765 102.136849,19.3445445 L102.136849,28.8124124 L99.0826868,28.8124124 L99.0826868,20.0368368 C99.0826868,18.4840841 98.5820967,16.7407407 96.1944507,16.7407407 C94.0261645,16.7407407 92.3331576,18.2626627 92.3331576,20.6646647 L92.3331576,28.7927928 L89.2705587,28.8124124 Z};
    \fill[#1] svg {M111.11091,29.1459459 C108.138305,29.1459459 105.719724,28.008008 104.333258,25.8778779 L106.498732,24.355956 C107.609592,25.9059059 109.386968,26.6514515 111.279648,26.6514515 C113.085148,26.6514515 114.3085,25.9871872 114.3085,24.7147147 C114.3085,23.3861862 112.975468,23.1087087 110.613132,22.7219219 C107.550534,22.194995 105.109454,21.3373373 105.109454,18.3383383 C105.109454,15.3393393 107.803641,13.9351351 110.832492,13.9351351 C113.776974,13.9351351 115.917137,15.2104104 117.112367,16.4828829 L115.166252,18.2542543 C114.043987,17.0478012 112.454477,16.3818701 110.804369,16.4268268 C109.415091,16.4268268 108.082059,16.9257257 108.082059,18.0608609 C108.082059,19.3361361 109.637263,19.6108108 111.555254,19.9443443 C114.665662,20.5049049 117.334539,21.3009009 117.334539,24.3727728 C117.334539,27.2344344 115.000326,29.1459459 111.11091,29.1459459 Z};
    \fill[#1] svg {M120.054036,9.04424424 L123.111011,9.04424424 L123.111011,25.0202202 C123.111011,26.2086086 123.611601,26.5421421 124.387797,26.5421421 C124.824414,26.5496047 125.255542,26.4443594 125.639272,26.2366366 L126.221419,28.562963 C125.493208,28.9372015 124.680714,29.1186471 123.861896,29.0898899 C122.500741,29.0898899 121.330822,28.6750751 120.667119,27.7613614 C120.194652,27.0690691 120.054036,26.2646647 120.054036,24.9921922 L120.054036,9.04424424 Z};
    \fill[#1] svg {M140.673848,29.0338338 C139.312693,29.0338338 138.061218,28.3975976 137.757489,26.8728729 C136.56226,28.590991 134.618958,29.1459459 132.895016,29.1459459 C129.894288,29.1459459 127.894739,27.5119119 127.894739,24.6614615 C127.894739,21.0626627 131.089517,20.5077077 133.589655,20.233033 C135.701695,20.0116116 137.285022,19.8182182 137.285022,18.4056056 C137.285022,16.992993 135.673572,16.5501502 134.312417,16.5501502 C132.680057,16.568857 131.09167,17.0799188 129.756485,18.016016 L128.533132,15.7205205 C130.313927,14.5399521 132.409979,13.9207806 134.54865,13.9435435 C137.993723,13.9435435 140.409492,15.3281281 140.409492,18.8176176 L140.409492,25.435035 C140.409492,26.3767768 140.716033,26.7635636 141.438795,26.7635636 C141.719738,26.7749788 141.998299,26.7080003 142.243114,26.5701702 L142.577778,28.6750751 C141.973345,28.9195092 141.326102,29.0414697 140.673848,29.0338338 Z M137.313145,21.0878879 C136.469454,22.1389389 135.229228,22.1389389 133.674024,22.3883884 C132.11882,22.6378378 130.979837,23.0806807 130.979837,24.6026026 C130.979837,26.1245245 132.144131,26.7635636 133.645901,26.7635636 C135.56108,26.7635636 137.301896,25.7377377 137.301896,23.3021021 L137.313145,21.0878879 Z};
    \fill[#1] svg {M153.368588,28.0640641 C152.364995,28.8019644 151.141994,29.1829227 149.895392,29.1459459 C148.118016,29.1459459 146.756861,28.562963 145.958167,27.2904905 C145.457577,26.5421421 145.263528,25.6564565 145.263528,24.2438438 L145.263528,16.6286286 L142.816824,16.6286286 L142.816824,14.2770771 L145.263528,14.2770771 L145.263528,10.3727728 L148.357062,10.3727728 L148.357062,14.2770771 L152.856748,14.2770771 L152.856748,16.6286286 L148.328939,16.6286286 L148.328939,24.2718719 C148.328939,25.7377377 149.023578,26.43003 150.297552,26.43003 C150.964191,26.435647 151.612176,26.2108071 152.131174,25.7937938 L153.368588,28.0640641 Z};
    \fill[#1] svg {M168.841883,22.3071071 L157.730471,22.3071071 C157.868274,24.9641642 159.617527,26.43003 162.202034,26.43003 C163.806353,26.4533756 165.343187,25.7876222 166.42049,24.6026026 L168.420038,26.5141141 C166.892957,28.1201201 164.862473,29.1459459 162.086729,29.1459459 C157.16801,29.1459459 154.4457,25.9059059 154.4457,21.6148148 C154.4457,17.3237237 157.196133,13.9435435 161.780188,13.9435435 C166.198318,13.9435435 168.892505,17.0742743 168.892505,21.2532533 C168.895171,21.6052 168.878271,21.9570237 168.841883,22.3071071 Z M165.813032,20.0900901 C165.59086,17.6544545 163.897853,16.4072072 161.813936,16.4072072 C159.507847,16.4072072 157.952643,17.9319319 157.783905,20.0900901 L165.813032,20.0900901 Z};
    \fill[#1] svg {M182.231262,28.8124124 L182.231262,26.6794795 C181.105049,28.2654339 179.26158,29.1898321 177.312542,29.1459459 C173.175643,29.1459459 170.619259,25.8498498 170.619259,21.5587588 C170.619259,17.2676677 173.175643,13.9435435 177.312542,13.9435435 C179.262187,13.8940092 181.107783,14.8184222 182.231262,16.4072072 L182.231262,9.04424424 L185.324796,9.04424424 L185.324796,28.8124124 L182.231262,28.8124124 Z M177.981871,16.6846847 C175.203315,16.6846847 173.870282,18.8736737 173.870282,21.5587588 C173.870282,24.2438438 175.203315,26.4048048 177.981871,26.4048048 C180.760427,26.4048048 182.231262,24.2438438 182.231262,21.5587588 C182.231262,18.8736737 180.757615,16.6846847 177.981871,16.6846847 Z};
    \fill[#1] svg {M19.8066541,2.88928929 C29.1444475,2.88928929 36.7142247,10.4334929 36.7142247,19.7397397 C36.7142247,29.0459866 29.1444475,36.5901902 19.8066541,36.5901902 C10.4688607,36.5901902 2.89908349,29.0459866 2.89908349,19.7397397 C2.90993167,10.4379749 10.4733579,2.90010082 19.8066541,2.88928929 Z M19.8066541,0.12012012 C8.93430649,0.12012012 0.120527307,8.90412303 0.120527307,19.7397397 C0.120527307,30.5753565 8.93430649,39.3593594 19.8066541,39.3593594 C30.6790017,39.3593594 39.4927809,30.5753565 39.4927809,19.7397397 C39.4927809,8.90412303 30.6790017,0.12012012 19.8066541,0.12012012 Z};
    \fill[#1] svg {M24.5622599,27.9771772 C23.5662697,28.7102136 22.3519383,29.0882867 21.1143754,29.0506507 C19.3482486,29.0506507 17.9955304,28.4732733 17.1940239,27.2092092 C16.6990584,26.4664665 16.5050094,25.5863864 16.5050094,24.1821822 L16.5050094,16.6146146 L12.9643189,16.6146146 L12.9643189,14.2826827 L16.5050094,14.2826827 L16.5050094,10.4036036 L19.5676083,10.4036036 L19.5676083,24.2242242 C19.5676083,25.6816817 20.2566227,26.3683684 21.536221,26.3683684 C22.1973213,26.372111 22.8396617,26.1494861 23.3557815,25.7377377 L24.5622599,27.9771772 Z};
    \fill[#1] svg {M23.1476711,15.4206206 C23.143927,14.9471026 23.3290859,14.4914979 23.6624117,14.1540419 C23.9957375,13.8165859 24.4499237,13.6249234 24.9250471,13.6212212 L24.9812932,13.6212212 C25.4564165,13.6249234 25.9106027,13.8165859 26.2439286,14.1540419 C26.5772544,14.4914979 26.7624132,14.9471026 26.7586692,15.4206206 C26.7649056,16.405583 25.9695837,17.2095054 24.9812932,17.2172172 L24.9250471,17.2172172 C23.9367565,17.2095054 23.1414347,16.405583 23.1476711,15.4206206 Z};
    \fill[#1] svg {M188.229906,26.987788 C188.229906,25.994007 189.038255,25.188388 190.035405,25.188388 C191.032555,25.188388 191.840904,25.994007 191.840904,26.987788 C191.840904,27.981569 191.032555,28.787187 190.035405,28.787187 C189.038255,28.787187 188.229906,27.981569 188.229906,26.987788 Z};
  \end{tikzpicture}%
  \endgroup}


==> figures/logos/translated-mark.tex <==
\newcommand{\TranslatedMark}[2][black]{%
  \begingroup
  \pgfmathsetmacro{\tmarkscale}{(#2)/40}%
  \begin{tikzpicture}[x=1pt, y=1pt, xscale=\tmarkscale, yscale=-\tmarkscale]
    \useasboundingbox (0,0) rectangle (40,40);
    \fill[#1] svg {M19.8066541,2.88928929 C29.1444475,2.88928929 36.7142247,10.4334929 36.7142247,19.7397397 C36.7142247,29.0459866 29.1444475,36.5901902 19.8066541,36.5901902 C10.4688607,36.5901902 2.89908349,29.0459866 2.89908349,19.7397397 C2.90993167,10.4379749 10.4733579,2.90010082 19.8066541,2.88928929 Z M19.8066541,0.12012012 C8.93430649,0.12012012 0.120527307,8.90412303 0.120527307,19.7397397 C0.120527307,30.5753565 8.93430649,39.3593594 19.8066541,39.3593594 C30.6790017,39.3593594 39.4927809,30.5753565 39.4927809,19.7397397 C39.4927809,8.90412303 30.6790017,0.12012012 19.8066541,0.12012012 Z};
    \fill[#1] svg {M24.5622599,27.9771772 C23.5662697,28.7102136 22.3519383,29.0882867 21.1143754,29.0506507 C19.3482486,29.0506507 17.9955304,28.4732733 17.1940239,27.2092092 C16.6990584,26.4664665 16.5050094,25.5863864 16.5050094,24.1821822 L16.5050094,16.6146146 L12.9643189,16.6146146 L12.9643189,14.2826827 L16.5050094,14.2826827 L16.5050094,10.4036036 L19.5676083,10.4036036 L19.5676083,24.2242242 C19.5676083,25.6816817 20.2566227,26.3683684 21.536221,26.3683684 C22.1973213,26.372111 22.8396617,26.1494861 23.3557815,25.7377377 L24.5622599,27.9771772 Z};
    \fill[#1] svg {M23.1476711,15.4206206 C23.143927,14.9471026 23.3290859,14.4914979 23.6624117,14.1540419 C23.9957375,13.8165859 24.4499237,13.6249234 24.9250471,13.6212212 L24.9812932,13.6212212 C25.4564165,13.6249234 25.9106027,13.8165859 26.2439286,14.1540419 C26.5772544,14.4914979 26.7624132,14.9471026 26.7586692,15.4206206 C26.7649056,16.405583 25.9695837,17.2095054 24.9812932,17.2172172 L24.9250471,17.2172172 C23.9367565,17.2095054 23.1414347,16.405583 23.1476711,15.4206206 Z};
  \end{tikzpicture}%
  \endgroup}

